Degradation Alchemy: Self-Supervised Unknown-to-Known Transformation for Blind Hyperspectral Image Fusion

Hyperspectral image (HSI) fusion is an efficient technique that combines low-resolution HSI (LR-HSI) and high-resolution multispectral images (HR-MSI) to generate high-resolution HSI (HR-HSI). Existing supervised learning methods (SLMs) can yield promising results when test data degradation matches the training ones, but they face challenges in generalizing to unknown degradations. To unleash the potential and generalization ability of SLMs, we propose a novel self-supervised unknown-to-known degradation transformation framework (U2K) for blind HSI fusion, which adaptively transforms unknown degradation into the same type of degradation as those handled by pre-trained SLMs. Specifically, the proposed U2K framework consists of: (1) spatial and spectral Degradation Wrapping (DW) modules that map HR-HSI to unknown degraded HR-MSI and LR-HSI, and (2) Degradation Transformation (DT) modules that convert these wrapped data into predefined degradation patterns. The transformed HR-MSI and LR-HSI pairs are then processed by a pre-trained network to reconstruct the target HR-HSI. We train the U2K framework in a self-supervised manner using consistency loss and greedy alternating optimization, significantly improving the flexibility of blind HSI fusion. Extensive experiments confirm the effectiveness of our proposed U2K framework in boosting the adaptability of five existing SLMs under various degradation settings and surpassing state-of-the-art blind methods.

==> figure_tex/deg_setings.tex <==
% \begin{figure}[t]
%     \centering
%     %   \subfloat[U2K training]{%
%         % \label{fig:U2K_training}
%         \includegraphics[height=180pt]{figure/degradation.png}%
%     %   }
%     %   \hfill
%     %   \subfloat[U2K strategy]{%
%     %     \label{fig:STF_two_pairs}
%     %     \includegraphics[height=90pt]{figure/method_diff_2.png}%
%     %   }
%     \caption{
%       Illustration of the degradations used in the experiments.
%     }
%     \label{fig:degradation}
% \end{figure}
\begin{figure}[t]
    \centering
        % \label{fig:U2K_training}
        \includegraphics[height=172pt]{figure_pdf/deg_setings_v9.pdf}%
    %   }
    %   \hfill
    %   \subfloat[U2K strategy]{%
    %     \label{fig:STF_two_pairs}
    %     \includegraphics[height=90pt]{figure/method_diff_2.png}%
    %   }
    \caption{
    % Baseline， C2F,U2K策略在不同退化设置下的表现。
    %   Illustration of the degradations used in the experiments.
      The performance of the baseline, C2F, and U2K strategies 
      under various degradation settings.
    }
    \label{fig:deg_setings}
    \vspace{-10pt}
  \end{figure}
